Hybrid Inlining: A Compositional and Context Sensitive Static Analysis Framework

Context sensitivity is essential for achieving the precision in inter-procedural static analysis. To be (fully) context sensitive, top-down analysis needs to fully inline all statements of the callees at each callsite, leading to statement explosion. Compositional analysis, which inlines summaries of the callees, scales up but often loses precision, as it is not strictly context sensitive. We propose a compositional and strictly context sensitive framework for static analysis. This framework is based on one key observation: a compositional static analysis often loses precision only on some critical statements that need to be analyzed context sensitively. Our approach hybridly inlines the critical statements and the summaries of non-critical statements of each callee, thus avoiding the re-analysis of non-critical ones. In addition, our analysis lazily summarizes the critical statements, by stopping propagating the critical statements once the calling context accumulated is adequate. Hybrid Inlining can be as precise as context sensitive top-down analysis. We have designed and implemented a pointer analysis based on this framework. It can analyze large Java programs from the Dacapo benchmark suite and industry in minutes. In our evaluation, compared to context insensitive analysis, Hybrid Inlining just brings 65% and 1% additional time overhead on Dacapo and industrial applications respectively.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> latex/sec.PLDIreview.tex <==
\section{PLDI'22 review and rebuttal}

\begin{verbatim}
PLDI 2022 Paper #287 Reviews and Comments
===========================================================================
Paper #287 Hybrid Inlining: A Compositional and Context Sensitive
Framework for Flow Insensitive Static Analysis


Review #287A
===========================================================================

Overall merit
-------------
3. Weak accept

Reviewer expertise
------------------
3. Knowledgeable

Paper summary
-------------
The authors describe a production level static analysis for Java that is
achieves high scalabilitiy by defining analyses in a compositional way 
(i.e., though summaries). Such an analysis also achieves precision since 
call site sensitivity is no longer required. The authors demonstrate how 
this analysis technique can be instantiated into pointer analysis and taint
analysis and evaluate their tool over the Dacapo benchmarks and other large
benchmarks.

Comments for author
-------------------
- From program analysis PoV, approach appears trivial at first
- Unclear how instance and static field mutations are modelled
+ Very strong evaluation
+ Deployed in production in a real world setting


Summary based program analyses, e.g., [1, 2] have been around and are 
indeed both scalable and precise. The problem with a lot of Java code, and 
the style in which developers code, however, is that in order to achieve 
good coverage of the program the state mutation (static and instance 
fields) need to be also modelled. Although this is not documentat so well 
in the paper, I am certain that the implemented tool does model this in 
some way however the *extent* to which this is modelled and the technique 
used would be the most interesting aspect of such work. One can infer this 
from the evaluation, as many methods wouldn't be reachable otherwise. 
Please explain this part of your analysis better in the next revision. 
Summary-based analyses for pure languages (the first 6 pages) is easy, and 
already adopted in several frameworks as a fallback or some preanalyses 
(including in Gigahorse and Wala).

Despite this, I understand that a production analysis needs to be fast and 
perhaps existing approaches that model state in a more principled way may 
still not be adaquate for the applications that the mentioned internet 
company requires and so there is still merit in the approach. The rest of 
the review offers some scattered concerns:

> We prove that compositional analysis with hybrid inlining is as precise 
as ∞-callsite sensitive global analysis.

This is well known, in the context of summary-based analyses for pure programs.


There are 3 distinct sections in this paper called "hybrid inlining" :)

Can you describe how your approach to modelling fields differs from access 
paths in the context of taint analysis?

How does your approach compare against Doop, P/Taint (e.g., for DaCapo)?

Can you include statistics about call graph edges in Table 1?


[1] Yan et al. Rethinking Soot for Summary-Based Whole-Program Analysis. 2012

[2] Schubert et al. PhASAR: An Inter-procedural Static Analysis Framework for C/C++



Review #287B
===========================================================================

Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
4. Expert

Paper summary
-------------
The paper proposes hybrid inlining, an approach that scales 
context-sensitive and flow insensitive bottom-up program analyses. The main
insight is that a major problem with bottom-up program analyses is that due
to lacking contexts, statements like function calls and field accesses 
cannot be precisely analyzed when  summaries. The key of idea 
of the paper is the analyses of such statements can be delayed until the 
contexts become sufficient to analyze them precisely. Around this idea, the
paper formalizes a general framework and instantiates a pointer analysis 
and a taint analysis. The paper evaluates the approach on the Dacapo suite 
and a set of Android apps, and show it outperforms existing approaches with
moderate overhead.

Comments for author
-------------------
I think this paper has interesting ideas and deserve publication at some 
point, but I am wondering whether it would benefit from another round of 
revision. 

In terms of the problem, bottom-up/compositional inter-procedural  program 
analyses have been less explored compared to their top-down counterpart 
(including call-string-based approaches). While having the property of 
being modular, it is often hard to construct summaries as without knowing 
the contexts, the situations can be too many. So the problem has both 
scientific values and practical values.

The paper proposes a simple yet elegant solution. The main idea is that we 
can do our best to summarize the statements that are not affected by the 
unknown contexts  and deal with the others when the contexts are 
sufficient. The paper formalizes a framework, which I find adequate. 
Although it might seem obvious to the authors, I would still like to see a 
soundness theorem.

I feel the paper could be improved in the following ways:

1. It is not quite clear to me which class of analyses the framework can be 
applied to. Is there any particular reason to limit the framework to 
flow-insensitive analyses? Is it because the transfer functions are usually
monotone? Also, in terms of instantiation, the pointer analysis and the 
taint analysis are very similar. I would like to see applications to other 
analyses which are not so similar.

2. How to improve the scalability/precision of context-sensitive pointer 
analyses is a very active field. There are many methods, especially ones 
that selectively increases the contexts. I would like to see emprical 
comparison with one of recent works. Without seeing the evidence, it is 
hard to me to estimate how much it improves existing approaches in 
practice. Just to give a few references (there are many more):

Tan, T., Li, Y., Ma, X., Xu, C. and Smaragdakis, Y., 2021. Making pointer 
analysis more precise by unleashing the power of selective context 
sensitivity. Proceedings of the ACM on Programming Languages, 5(OOPSLA), 
pp.1-27.

Jeon, M., Jeong, S. and Oh, H., 2018. Precise and scalable points-to 
analysis via data-driven context tunneling. Proceedings of the ACM on 
Programming Languages, 2(OOPSLA), pp.1-29.

Zhang, X., Mangal, R., Grigore, R., Naik, M. and Yang, H., 2014, June. On 
abstraction refinement for program analyses in Datalog. In Proceedings of 
the 35th ACM SIGPLAN Conference on Programming Language Design and 
Implementation (pp. 239-248).

Questions:
1. How do you handle recursions?
2. What are the android applications in the experiment?
3. I think the optimizations in Section 5 affect the precision? How do you 
expect people to choose them in practice?

Minor:

I am not sure if we can infer much from the data in Table 4 as both 
analyses are unsound.



Review #287C
===========================================================================

Overall merit
-------------
3. Weak accept

Reviewer expertise
------------------
3. Knowledgeable

Paper summary
-------------
For context-sensitive analysis, global top-down analysis and
compositional bottom-up analysis have well-known their own pros and
cons.  Based on an observation that a compositional static analysis
often loses precision only on some "critical" statements with the
absence of context, this paper proposes a compositional and
strictly context sensitive framework for flow insensitive analysis.
By distinguishing statements between critical ones and non-critical
ones, the proposed approach inlines critical ones and summarized
non-critical ones of each callee, and summarizes critical ones with
the context from callers in a lazy manner.  The authors implemented a
pointer analysis and a taint analysis in the proposed framework, which
can analyze large Java programs as fast as context insensitive analysis.

Comments for author
-------------------
This paper proposes a hybrid approach for compositional static
analysis in the sense that a flow-insensitive static analysis utilizes
both a top-down approach and a bottom-up approach depending on
critical and non-critical statements.  The main analysis basically
takes a bottom-up approach to define each function's summary, but
it defers the analysis of critical statements till when it can analyze
them precisely.

The key idea of this hybrid inlining is to define Context Ready
Predicate (CRP), the function that determines when to analyze criticall
statements precisely, in a parametric manner.  While the CRP can be
defined based on k-CFA, the authors instead define CRP that is exactly
apposite of the definition of critical statements and extend the CRP
for adequate contexts, and proved that the hybrid inlining using both
CRPs have the exactly same precision with an infinite-sensitive
top-down analysis.  Theorem 3.2 in page 6 shows that but only for
monotone abstract transfer functions.

The main contribution of the paper is to define the following concepts
in a high level:

	- critical statements
	- hybrid summary (hybrid inlining)
	- context ready predicate
	- adequate context

and explain how the proposed hybrid approach is different from the
traditional bottom-up appraoch using examples.  In addition, the paper
empirically shows that the proposed approach is a bit slower than the
traditional bottom-up approach but improves the analysis precision much.

It would make the paper stronger if it compares the proposed approach
with realted work in more detail.  While there exist many hybrid
approaches between top-down and bottom-up analyses, the paper simply
emphasizes that this is the first attempt for flow-insensitive analysis.

It would be interesting to apply the proposed approach to different
programming languages by defining language-specific critical
statements well.  That may lead to similarly fast analysis with
reasonable precision.



Review #287D
===========================================================================

Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
4. Expert

Paper summary
-------------
The paper presents a compositional context-sensitive analysis technique via
hybrid inlining. They identify the statements whose summarization can be 
affected by the context information. These statements are called critical 
statements. During the compositional analysis, they hybridly inline the 
critical statements and the summarizaiton of non-critical statements, thus 
avoiding the re-analysis of non-critical ones. For the sake of further 
optimization, they stop propagating the critical statements once the 
calling context accumulated is adequate. In this case, the critical 
statements are summarized as well in a lazy way. 

The framework is implemented and employed in industry to analyze real-world 
large-scale programs. Baed on the framework, two client analyses, pointer 
analysis and taint analysis are developed. The experimental evaluations 
show that the pointer analysis via hybrid inlining proposed runs as fast as
context-insenstive analysis while achieving higher precision than 
context-insensitive analysis. The taint analysis with hybrid inlining 
outperforms Flowdroid and context-insenstive taint analysis in terms of 
both precision and recall.

Comments for author
-------------------
Thanks for submitting the work to PLDI. The paper targets a relevant static
analysis problem which is to achieve the context-sensitivity in a both 
precise and scalable way. 

Based on the insight that the compositional analysis loses precision only 
on certain critical statements in the absense of context, the hybrid 
inlining of statements is proposed. To be honest, I appreciate the idea. In
essence, it is a kind of selective context sensitivity at the granularity 
of statements. 

My concern mainly comes from the evaluation which is far from being 
complete as a PLDI paper. Although as claimed, the non-critical statements 
can be prevented from being re-analyzed, it is still hard to determine the 
advantage against the state-of-the-art approaches empiricially. As a 
candidate selective context sensitivitive analysis, it is necessary to 
compare with the state-of-the-art approaches (e.g., [22,25,26]) to measure 
its effectiveness with respect to both performance and precision.

Moreover, I have the following questions and comments. 
- How do you determine the critical statements given a program to be analyzed?
- Is that possible to extend this technique to other languages, like C/C++?
What should be adapted?
- All the figures and tables should be self-interpreted. 
- minor typo: line 500, "may lose? precision..."




=============rebuttal================

We thank the reviewers for their thoughtful comments. We address the common questions and selected relevant specific questions in the first 700 words and other questions after 700 words. For questions about algorithmic details that cannot be fully addressed, please refer to our implementation, which will be open-sourced.

Common Questions

Question: No experimental comparison with top-down selectively context sensitive analysis?

Response: We indeed have compared our work with a top-down selectively context sensitive analysis: FlowDroid. FlowDroid utilizes a demand-driven alias analysis, which restores context sensitivity on pointers when needed. Different from [1][2][3] which relies on a pre-analysis to select context sensitivity, FlowDroid does that on the fly. The experimental results show that our tool significantly out-performs FlowDroid on precision and performance.

We choose FlowDroid over other recent works [1][2][3] (which are implemented within Soot and Doop) because: (1) FlowDroid is still among the best available taint analyzers [5]. P/Taint[7] with selective context sensitivity from Doop does not show better experimental results; (2) While “Running Soot, WALA, or Doop out of the box on a realistic Java enterprise application yields virtually zero coverage of the application code, or fails to scale”[4], FlowDroid is recently reported [6] to be able to run on real enterprise applications.

Our implementation can stably (i.e., more than 90% tasks can be finished within 10 minutes) analyze the Dacapo suite and industrial applications with at least 4-call-site sensitivity (\infty∞-call-site sensitivity in most cases). This is way beyond the reported ability of [1][2][3], where the highest achieved context sensitivity is within 33-obj/callsite sensitivity on the same Dacapo suite, with hours of time consumption.

Question: Why only applying hybrid inlining to flow-insensitive analysis ?

Response: Hybrid inlining can be applied to flow-sensitive analysis. However, it is not practical. In flow sensitive analysis, each program point (before and after each statement) is associated with an abstract state. As a result, in a hybrid summary with nn critical statements, we need to store n+1n+1 abstract states. This raises serious performance concern. In contrast, a flow-insensitive analysis just needs to maintain one global abstract state. We will elaborate this in the revised version.

Selected Specific Questions

Reviewer B

Question: How is hybrid inlining applied on other analysis?

Response: Hybrid inlining can be instantiated with any bottom-up analysis, e.g., a bottom-up string analysis, where critical statements are string manipulation statements.

Question: Table 4 shows both analyses are unsound.

Response: Actually our hybrid inlining algorithm is sound. However, in practice, we have to model the behaviors of J2EE frameworks (e.g. Spring), like [4]. In this case, the soundness of the static analyzer depends on whether all behaviors of the framework are taken into account. The missed source-sink pairs by our tool are actually caused by Spring Interceptors. We do not model this because developers claim that, the data propagated with Interceptors are usually not important.

Question: How to handle recursions?

Response: For recursions on call strings, our analysis just over-approximates all invocation statements in the second occurrence of a method. However, this process is not simple in practice. First, we never put abstract methods in the call string to avoid false recursions; Second, we have to deal with many corner cases. For instance, if an abstract method A has nn implementations, each of which invokes the abstract method A. There could be at most n!n! (i.e., factorial of nn) call strings without recursion. There are other corner cases like this permutation explosion. We have developed some benchmarks specially for recursion, and are happy to contribute them to the community. The case for access string is similar.

Reviewer C

Question: Difference with other hybrid top-down and bottom-up analysis?

Response: Our analysis is actually not a hybrid top-down and bottom-up analysis. It is a one-pass bottom-up analysis without a pre-computed call graph. The hybrid in the name indicates that the summary is hybrid.

Reviewer D

Question: Application to other languages? How to determine the critical statements given a program?

Response: Our framework applies to other languages. Critical statements depend on the specific analysis and languge. For pointer analysis on C++, critical statements will be virtual invocation, container access and function pointer deference. They can be picked out by simple syntactic checking during analysis.

Other Specific Questions

Reviewer A

Question: How fields are modeled?

Response: Memory model itself is an important topic. We will elaborate this a bit in the revised version. For more details, please refer to our implementation.

Question: How does your approach compare against Doop, P/Taint (e.g., for DaCapo)?

Response: To us, P/Taint is a similar tool with FlowDroid. It does not out-perform FlowDroid from the experimental results reported in their paper. On Dacapo, it is too hard to get oracle for taint analysis. On industrial applications, oracle is easier to get with the help of developers. This explains why we conduct comparison with FlowDroid on industrial applications.

Reviewer B

Question: I think the optimizations in Section 5 affect the precision? How do you expect people to choose them in practice?

Response: The optimizations only lose precision in some extreme cases. They are from our experience in applying our tool on hundreds of real applications from the company and on the open source test case suite Dacapo. For most people, they can just take all the optimizations.

Question: What are the android applications in the experiment?

Response: They are J2EE applications that are practically in use in the Internet Company, not Android applications. We have to anonymize the names as the company requests. These applications focus on financial transactions.

Reviewer C&D

All other questions have been answered in the common question part.

[1]Yue Li, Tian Tan, Anders Møller, and Yannis Smaragdakis. 2020. A principled approach to selective context sensitivity for pointer analysis.ACM Transactions on Programming Languages and Systems (TOPLAS)42, 2 (2020), 1–40.

[2]Jingbo Lu and Jingling Xue. 2019. Precision-preserving yet fast object-sensitive pointer analysis with partial context sensitivity.Proceedingsof the ACM on Programming Languages3, OOPSLA (2019)

[3] Tan, Tian, Yue Li, Xiaoxing Ma, Chang Xu, and Yannis Smaragdakis. "Making pointer analysis more precise by unleashing the power of selective context sensitivity." Proceedings of the ACM on Programming Languages 5, no. OOPSLA (2021): 1-27

[4] Antoniadis, Anastasios, Nikos Filippakis, Paddy Krishnan, Raghavendra Ramesh, Nicholas Allen, and Yannis Smaragdakis. "Static analysis of Java enterprise applications: frameworks and caches, the elephants in the room." In Proceedings of the 41st ACM SIGPLAN Conference on Programming Language Design and Implementation, pp. 794-807. 2020.

[5] Pauck, Felix, Eric Bodden, and Heike Wehrheim. "Do android taint analysis tools keep their promises?." In Proceedings of the 2018 26th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering, pp. 331-341. 2018.

[6] Jie Wang, Yunguang Wu, Gang Zhou, Yiming Yu, Zhenyu Guo, andYingfei Xiong. 2020. Scaling static taint analysis to industrial SOA ap-plications: a case study at Alibaba. InProceedings of the 28th ACM JointMeeting on European Software Engineering Conference and Symposiumon the Foundations of Software Engineering. 1477–1486.

[7] Grech, Neville, and Yannis Smaragdakis. "P/taint: Unified points-to and taint analysis." Proceedings of the ACM on Programming Languages 1, no. OOPSLA (2017): 1-28.

\end{verbatim}


==> latex/sec.implementation.tex <==
\presec
\section{Implementation} \label{sec:implementation}
\postsec

We have implemented our pointer analysis with \toolname in Java based on GraalVM~\cite{graalvm}. 
Both  are industrial grade implementations targeting at thousands of real applications in
an Internet company.  
% Most of these applications are in Java 8 and deployed as microservices. 
% Each application has usually between 100K lines and 1 million lines of code with a heavy use of libraries and frameworks like Spring~\cite{springCloud}. 
% We have modeled the most relevant behaviors of the frameworks (RPC and HTTP service entrances, Database accesses, Beans, messages, dynamic configurations \etc) and libraries (Lambda functions, operations on Json/Map/List, String, Date, \etc).

In our implementation, the context ready predicate \(\predcrit\) is set to be adequate  with the following optimizations:
 \begin{itemize}
    \item[\bf Opt1:] If the virtual invocation statements from the same class appear more than a threshold in a hybrid summary, our analysis limits their propagation steps to be \(k\)-callsite sensitive on those individual statements;
    \item[\bf Opt2:] If the receiver of a virtual invocation statement is from the iteration result over a container, our analysis does not propagate this virtual invocation statement further;
    \item[\bf Opt3:] Permutation explosion is killed whenever detected. 
\end{itemize}

 These optimizations come from our experience applying our work in the industry.  Opt1 tackles the case where programmers use a visitor-like style, by which an object is passed as a parameter through many procedures and  used heavily as the receivers of many  virtual invocation statements. This causes the number of critical statement to explode. By adjusting \(k\) on individual statements dynamically, we gain flexibility in trading off precision and performance. We never set \(k\) under 4 except for ``eclipse'' where  $k=3$   since it uses visitors extensively.  Opt2 comes from our observation that there is usually no precision  gain with further propagation in that case.  Opt3 is slightly more complex. In Section~\ref{recursion}, our analysis detects recursion by finding the re-occurrences of some callsite in the call string. However, this does not avoid permutation explosion. For instance, consider a polymorphic procedure  in an interface with $n$ different implementations in $n$ different classes, with each calling the polymorphic procedure on receiver objects from these
 classes. Then there are potentially  $n!$ non-recursive call strings. Our analysis avoids this permutation explosion by passing the set of non-deterministic polymorphic callsites together with the call string. On detecting that a polymorphic procedure is dispatched to more than $m$ implementations multiple times in a call string, our analysis will just return an approximation of it. Here, $m$ is parametric. We set $m=5$ by default. 
 %The same phenomenon can also be observed on field access paths. Our analysis avoids recursion and permutation explosion in a similar way. 
 This can result in some precision loss, serves to make sure that the analysis terminates. 

 

% \subsection{GraalVM}
% \subsection{Pointer Analysis}
% \subsection{Taint Analysis}
